I2V-Adapter: A General Image-to-Video Adapter for Diffusion Models

Text-guided image-to-video (I2V) generation aims to generate a coherent video that preserves the identity of the input image and semantically aligns with the input prompt. Existing methods typically augment pretrained text-to-video (T2V) models by either concatenating the image with noised video frames channel-wise before being fed into the model or injecting the image embedding produced by pretrained image encoders in cross-attention modules. However, the former approach often necessitates altering the fundamental weights of pretrained T2V models, thus restricting the model's compatibility within the open-source communities and disrupting the model's prior knowledge. Meanwhile, the latter typically fails to preserve the identity of the input image. We present I2V-Adapter to overcome such limitations. I2V-Adapter adeptly propagates the unnoised input image to subsequent noised frames through a cross-frame attention mechanism, maintaining the identity of the input image without any changes to the pretrained T2V model. Notably, I2V-Adapter only introduces a few trainable parameters, significantly alleviating the training cost and also ensures compatibility with existing community-driven personalized models and control tools. Moreover, we propose a novel Frame Similarity Prior to balance the motion amplitude and the stability of generated videos through two adjustable control coefficients. Our experimental results demonstrate that I2V-Adapter is capable of producing high-quality videos. This performance, coupled with its agility and adaptability, represents a substantial advancement in the field of I2V, particularly for personalized and controllable applications.

==> figs/fig_i2v_control_figonly.tex <==
\begin{figure*}%[p]
   \setlength{\abovecaptionskip}{5pt}
    \centering
    \includegraphics[width=\linewidth]{figure/revision_controlnet_v3_cropped.pdf}
    \caption{Our results with ControlNet~\cite{controlnet}. The pose control is shown as an inset at the bottom left for each frame.}
\label{fig:i2v_control}
\end{figure*}


==> figs/fig_i2v_dreambooth_figonly.tex <==
\begin{figure*}%[p]
%    \setlength{\abovecaptionskip}{5pt}
    \centering
    \includegraphics[width=\linewidth]{figure/revision_dreambooth_v2_cropped.pdf}
    \caption{Our results with personalized T2I models~\cite{DreamBooth}.}
\label{fig:i2v_dreambooth}
\end{figure*}


==> figs/fig_teaser.tex <==
\begin{teaserfigure}
	\includegraphics[width=0.99\textwidth]{figure/teaser_0123.pdf}
	\caption{
	\label{fig:teaser}
        Our lightweight I2V-Adapter achieves high-quality and versatile image-to-video generation, \textit{without tuning any pretrained spatial or temporal modules}. \textbf{{First row:}} I2V results of I2V-Adapter. \textbf{{Second row:}} results of I2V-Adapter combined with a personalized T2I model (\href{https://civitai.com/models/28169/cuteyukimixadorable-style?modelVersionId=265102}{\textit{CuteYukiMix}}). \textbf{{Third row:}} results of I2V-Adapter combined with ControlNet~\cite{controlnet}.
    }
	\Description[TeaserFigure]{TeaserFigure}
\end{teaserfigure}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sections/3_1_preliminary_LDM.tex <==
Given a data $\mathbf{x}_0\sim p_\mathrm{data}(\mathbf{x})$, the forward process gradually adds Gaussian noise $\gaussiannoise\sim\mathcal{N}(\boldsymbol{0},\boldsymbol{1})$ to the data to obtain a noised data, as shown as follows:
\begin{equation}
    \mathbf{x}_t = \alpha_t\mathbf{x}_0 + \sigma_t\gaussiannoise,
\end{equation}
where $\alpha_t,\sigma_t\in[0,1]$ are two predefined functions of random time step $t\sim \mathcal{U}({1,\dots,T})$, satisfying the variance preserving principle, \ie, $\alpha_t^2 + \sigma_t^2=1$.

Diffusion models typically train a neural network $\neuralnetwork(\cdot)$ to learn the added noise, which is denoised during sampling to gradually generate new data.
For any condition $\mathbf{c}$ (\eg, text, image, and audio), the training objective function is defined as
\begin{equation}
    \min_{\theta} \mathbb{E}_{\mathbf{x}_0,\mathbf{c},t,\gaussiannoise}\left[\|\gaussiannoise-\neuralnetwork(\mathbf{x}_t,\mathbf{c},t)\|_2^2\right].
\end{equation}

For sample generation, diffusion models first sample a Gaussian noise, then progressively denoise it to obtain the final generated result (Eq.~\ref{eq:sampling}). Furthermore, this Markov sampling process can be accelerated by methods like DDIM~\cite{song2020denoising}:
\begin{equation}\label{eq:sampling}
    \mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}}\left(\mathbf{x}_t-\frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}}\neuralnetwork(\mathbf{x}_t,\mathbf{c},t)\right)+\sigma_t\boldsymbol{\epsilon}.
\end{equation}

Classifier-free guidance sampling~\cite{ho2021cfg} enables flexible and controllable conditional generation of diffusion models. By training an unconditional diffusion model $\neuralnetwork(\mathbf{x}_t,t)$ and a conditional model $\neuralnetwork(\mathbf{x}_t,\mathbf{c},t)$ via a single neural network $\neuralnetwork$, we can redefine the conditional noise prediction as follows to gain flexible and controllable results,
\begin{equation}
    \hat{\neuralnetwork}(\mathbf{x}_t,\mathbf{c},t) = w \cdot \neuralnetwork(\mathbf{x}_t,\mathbf{c},t) + (1 - w) \cdot \neuralnetwork(\mathbf{x}_t,t),
\end{equation}
where $w\in\mathbb{R}^+$ is a user-specified hyperparameter.

